Esophageal Tumor Segmentation in CT Images using Dilated Dense Attention Unet (DDAUnet)

Manual or automatic delineation of the esophageal tumor in CT images is known to be very challenging. This is due to the low contrast between the tumor and adjacent tissues, the anatomical variation of the esophagus, as well as the occasional presence of foreign bodies (e.g. feeding tubes). Physicians therefore usually exploit additional knowledge such as endoscopic findings, clinical history, additional imaging modalities like PET scans. Achieving his additional information is time-consuming, while the results are error-prone and might lead to non-deterministic results. In this paper we aim to investigate if and to what extent a simplified clinical workflow based on CT alone, allows one to automatically segment the esophageal tumor with sufficient quality. For this purpose, we present a fully automatic end-to-end esophageal tumor segmentation method based on convolutional neural networks (CNNs). The proposed network, called Dilated Dense Attention Unet (DDAUnet), leverages spatial and channel attention gates in each dense block to selectively concentrate on determinant feature maps and regions. Dilated convolutional layers are used to manage GPU memory and increase the network receptive field. We collected a dataset of 792 scans from 288 distinct patients including varying anatomies with \mbox{air pockets}, feeding tubes and proximal tumors. Repeatability and reproducibility studies were conducted for three distinct splits of training and validation sets. The proposed network achieved a $\mathrm{DSC}$ value of $0.79 \pm 0.20$, a mean surface distance of $5.4 \pm 20.2mm$ and $95\%$ Hausdorff distance of $14.7 \pm 25.0mm$ for 287 test scans, demonstrating promising results with a simplified clinical workflow based on CT alone. Our code is publicly available via \url{https://github.com/yousefis/DenseUnet_Esophagus_Segmentation}.

==> anatomies/anatomies.tex <==


\begin{figure}[!tb]
\centering

\begin{tabular}{ccc}
      \includegraphics[height=22mm]{./anatomies/TEST022-1.png}&
      \includegraphics[height=22mm]{./anatomies/TEST022-2.png}&      \includegraphics[height=22mm]{./anatomies/TEST022-3.png} \\
      \includegraphics[height=22mm]{./anatomies/LBAL-1.png} &
      \includegraphics[height=22mm]{./anatomies/LBAL-2.png} &
      \includegraphics[height=22mm]{./anatomies/LBAL-3.png}  \\
       \includegraphics[height=22mm]{./anatomies/TEST078-1.png} &
      \includegraphics[height=22mm]{./anatomies/TEST078-2.png} &
      \includegraphics[height=22mm]{./anatomies/TEST078-3.png} \\
\end{tabular}
% \begin{tikzpicture}
% \node [anchor=west] (water) at (-1,1) {\Large Water};
% \begin{scope}[x={(image.south west )},y={(image.north east)}]
% \draw [-stealth, line width=5pt, cyan] (water) -- ++(0.4,0.0);
% \end{scope}
% \end{tikzpicture}%
% \begin{tikzpicture}[
%     x={(-0.3cm,-0.2cm)}, y={(0.6cm,-0.1cm)}, z={(0cm,.5cm)}% x-y grid is wacky
%     ]
%     \hspace*{-.5in}

%     \put(120,160){\drasre{0}{3}{0}{3}{0}{3}}

%   \end{tikzpicture}
  
\caption{Axial, coronal and sagittal view of some challenging cases, from up to down: a patient with an air packet inside the esophagus lumen, a patient with an air packet and a feeding tube inside the esophagus lumen, a patient with a tumor extened into the stomach. GTVs are surrounded by green contours. }\label{fig:challengingcases}
\end{figure}

% Hiatal hernia on thoracic computed tomography in pulmonary fibrosis
% http://erj.ersjournals.com/content/48/3/833.figures-only

==> figures/challengingcases.tex <==
\begin{figure*}[!tb]
\small
\centering
\begin{tabular}{ccccc}

    \rotatebox{90}{Patient$\#$1, DSC=0.42}& \includegraphics[height=30mm,width=35mm,trim={2cm 2cm 2cm 2cm},clip]{./challenging_cases/TEST108_bigextension1.png}&\includegraphics[height=30mm,width=35mm,trim={2cm 2cm 2cm 2cm},clip]{./challenging_cases/TEST108_bigextension2.png}&\includegraphics[height=30mm,width=35mm,trim={2cm 2cm 2cm 2cm},clip]{./challenging_cases/TEST108_bigextension3.png}&\includegraphics[height=30mm,width=35mm,trim={2cm 2cm 2cm 2cm},clip]{./challenging_cases/TEST108_bigextension4.png}\\
    
   \rotatebox{90}{Patient$\#$2, DSC=0.31}& \includegraphics[height=30mm,width=35mm,trim={2cm 2cm 2cm 2cm},clip]{./challenging_cases/TEST026_contrast1.png}&\includegraphics[height=30mm,width=35mm,trim={2cm 2cm 2cm 2cm},clip]{./challenging_cases/TEST026_contrast2.png}&\includegraphics[height=30mm,width=35mm,trim={2cm 2cm 2cm 2cm},clip]{./challenging_cases/TEST026_contrast3.png}&\includegraphics[height=30mm,width=35mm,trim={2cm 2cm 2cm 2cm},clip]{./challenging_cases/TEST026_contrast4.png}\\
   
   \rotatebox{90}{Patient$\#$3, DSC=0.60}& \includegraphics[height=30mm,width=35mm,trim={1cm 1cm 1cm 1cm},clip]{./challenging_cases/TEST099_feeding1.png}&\includegraphics[height=30mm,width=35mm,trim={1cm 1cm 1cm 1cm},clip]{./challenging_cases/TEST099_feeding2.png}&\includegraphics[height=30mm,width=35mm,trim={1cm 1cm 1cm 1cm},clip]{./challenging_cases/TEST099_feeding3.png}&\includegraphics[height=30mm,width=35mm,trim={1cm 1cm 1cm 1cm},clip]{./challenging_cases/TEST099_feeding4.png}\\
    

\end{tabular}
\caption{Results for some challenging cases, from top to bottom: a patient with a large extension of tumor in stomach, a patient with contrast agent and air pocket, a patient with a feeding tube and air pockets}\label{fig:challengingcases}
\end{figure*}

==> figures/failurecases.tex <==
\begin{figure*}[!tb]
\centering

\begin{tabular}{cccc}
    {DSC=0}&{DSC=0.03}&{DSC=0}&{DSC=0}\\
    \includegraphics[height=30mm,width=40mm]{./failure_cases/TEST086_lung_1.png}&\includegraphics[height=30mm,width=40mm]{./failure_cases/TEST033_variation_1.png}&\includegraphics[height=30mm,width=40mm]{./failure_cases/TEST034_haital_1.png}&\includegraphics[height=30mm,width=40mm]{./failure_cases/TEST097_fat_1.png}
    \\
    \includegraphics[height=30mm,width=40mm]{./failure_cases/TEST086_lung_2.png}&\includegraphics[height=30mm,width=40mm]{./failure_cases/TEST033_variation_2.png}&\includegraphics[height=30mm,width=40mm]{./failure_cases/TEST034_haital_2.png}&\includegraphics[height=30mm,width=40mm]{./failure_cases/TEST097_fat_2.png}
    \\
    \includegraphics[height=30mm,width=40mm]{./failure_cases/TEST086_lung_3.png}& \includegraphics[height=30mm,width=40mm]{./failure_cases/TEST033_variation_3.png}&\includegraphics[height=30mm,width=40mm]{./failure_cases/TEST034_haital_3.png} &\includegraphics[height=30mm,width=40mm]{./failure_cases/TEST097_fat_3.png} 
    \\
\end{tabular}
\caption{Some of the failure cases, for each case the ground truth and the network output are shown by green and red contours, receptively, from top to bottom: DSC value, axial, coronal and sagittal view, from left to right: a patient with contrast agent, variation in position due lung removal, variation in position, Hiatal hernia, variation for losing fat. }\label{fig:failurecases}
\end{figure*}

==> figures/overlaped_test.tex <==
%\documentclass{article}
%\usepackage{stackengine}
%\usepackage{graphicx}
\parskip 1em
%\begin{document}
\def\big{\includegraphics[height=4cm]{example-image}}
\def\little{\includegraphics[height=1.2cm]{example-image}}
\def\stackalignment{l}
\topinset{\little}{\big}{5pt}{2pt}
\bottominset{\little}{\big}{5pt}{25pt}\par
\def\stackalignment{r}
\topinset{\little}{\big}{7pt}{7pt}
\bottominset{\little}{\big}{12pt}{-5pt}
%\end{document}

==> figures/successfulcases.tex <==
%\def\Put(#1,#2)#3{\leavevmode\makebox(0,0){\put(#1,#2){#3}}}

\begin{figure*}[!tb]
\small
\centering
\begin{tabular}{cccc}

    {{Patient$\#$1, DSC=0.89}}& {{Patient$\#$2, DSC=0.89}}& {{Patient$\#$3, DSC=0.87}}& {{Patient$\#$4, DSC=0.78}}\\
    \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] at (0,0) 
    {\includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/RAWO_1.png}};
    %\Put(10,50) {\includegraphics[height=30mm,width=35mm,trim=10cm 10cm 11cm 11cm},clip]{./successful_cases/RAWO_1.png}};
   \draw[red,ultra thick] (1.3,1.0) rectangle (2.2,1.9);
    \end{tikzpicture}&
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/LCRU_1.png}&
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/LWWI_1.png}&
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/LPRO_1.png}\\
    
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/RAWO_2.png}&
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/LCRU_2.png}&
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/LWWI_2.png}&
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/LPRO_2.png}\\
    
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/RAWO_3.png}&
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/LCRU_3.png}&
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/LWWI_3.png}&
    \includegraphics[height=30mm,width=35mm,trim={0cm 0cm 0cm 0cm},clip]{./successful_cases/LPRO_3.png}\\
    
\end{tabular}
\caption{Successful cases, for each case the ground truth and the network output are shown by green and red contours and 3D-DSC values are reported, top to bottom: some slices. }\label{fig:successfulcases}
\end{figure*}


\def\stackalignment{l}
\topinset{\little}{\big}{5pt}{2pt}
\bottominset{\little}{\big}{5pt}{25pt}\par
\def\stackalignment{r}
\topinset{\little}{\big}{7pt}{7pt}
\bottominset{\little}{\big}{12pt}{-5pt}
